Machine Learning Techniques for Data Reduction of CFD Applications

We present an approach called guaranteed block autoencoder that leverages Tensor Correlations (GBATC) for reducing the spatiotemporal data generated by computational fluid dynamics (CFD) and other scientific applications. It uses a multidimensional block of tensors (spanning in space and time) for both input and output, capturing the spatiotemporal and interspecies relationship within a tensor. The tensor consists of species that represent different elements in a CFD simulation. To guarantee the error bound of the reconstructed data, principal component analysis (PCA) is applied to the residual between the original and reconstructed data. This yields a basis matrix, which is then used to project the residual of each instance. The resulting coefficients are retained to enable accurate reconstruction. Experimental results demonstrate that our approach can deliver two orders of magnitude in reduction while still keeping the errors of primary data under scientifically acceptable bounds. Compared to reduction-based approaches based on SZ, our method achieves a substantially higher compression ratio for a given error bound or a better error for a given compression ratio.

==> conclusion.tex <==








==> introduction.tex <==
Computational fluid dynamics (CFD) encompasses a broad range of  tools that enable the study of natural and engineered physical phenomenon that are critical to the nation’s energy security and economic competitiveness.  Direct numerical simulation (DNS) of turbulent combustion \cite{Chen2011,Vervisch2011, Driscoll2020,Apsden2011, Wen2023}, wherein all turbulence scales are numerically resolved, is enabling blends of hydrogen with natural gas and ammonia to be used in power generation \cite{rieth2023direct, rieth22, Wiseman2021}, and DNS of hypersonic flows is being used to predict aerodynamics around complex adaptive geometries in environments with strong thermal and chemical nonequilibrium \cite{desai2022effects, DESAI2023112681, Martin2011}. The  amount of data (as well as fidelity) generated from CFD simulations has increased enormously due to the availability of exascale supercomputers and is surpassing the extant storage, memory, and network capacities. The focus of this paper is to demonstrate the use of ML based autoencoders that encapsulate the following features:

\begin{compactenum}

\item	{\it Leverage Spatiotemporal Relationships in Mesh Structures:}  CFD  datasets have underlying data structures that consist of structured and block structured multidimensional meshes. It is important that the data reduction techniques address strong spatiotemporal correlations that are naturally present in these structures.
\item {\it Leverage Relationships within Tensors Representing Physics at Individual Grid Points:} CFD simulations update and store tensors comprised of several tens to a hundred species and their attributes at each grid point or particle. Reduction techniques should be able to leverage interrelationships between the elements of this tensor. Additionally, the values corresponding to each species may increase or decrease exponentially over the simulation.

\end{compactenum}

The proposed guaranteed block autonecoder (GBAE)  utilizes a multidimensional block of tensors in space and time to capture the spatio-temporal relationships as well as the interrelationships within the tensor. 
The original data are divided into smaller spatiotemporal blocks. a 3D convolutional autoencoder is utilized to capture the spatiotemporal correlations within each block. To guarantee the error bound of the reconstructed data, Principal Component Analysis (PCA) is applied to the residual between the original and reconstructed data. This yields a basis matrix, which is then used to project the residual of each instance. The resulting coefficients are retained to enable accurate recovery of the residual. The number of coefficients saved is incrementally increased until the error bound is satisfied. Additionally, quantization and entropy coding techniques are applied to both the latent data from the GAE and the PCA coefficients. This further improves the compression ratio of the overall process.



In addition, we show that differential reduction can be performed based on regions where a higher threshold of error is acceptable based on application requirements. We use lower error bounds on predicted critical regions and higher error bounds on the rest of space to ensure minimal false negatives on QoI and large compression ratios globally.
Currently, most state-of-the-art lossy compressors \cite{di2016fast, gong2022region, lindstrom2014fixed} are mostly focused on controlling global error such as $L^\infty$ and $L^2$. Without local error control, the application of differential compression requires the partitioning of ROIs and the rest of the data and compression of each part separately. In this paper, we employ a multilevel-decomposition-based compression method discussed in \cite{gong2022region} because it supports pixel-wise changed error bounds. The differentially compressed data can be reconstructed using the same algorithm and code as the uniformly compressed data. 



We validate our hybrid method using the simulation data generated by S3D. Provide details



In comparison to previous research \cite{SZ_3}, our method achieves a substantially higher compression ratio while also attaining a lower false negative (FN) ratio for both TC and AR detection, along with significantly improved quality of information preservation.


%


The rest of the paper is organized as follows. Section ~\ref{methodology} describes our compression pipeline. Experimental results using our method are presented in Section~\ref{expt}  for different levels of compression and accuracy. Section~\ref{relwork} presents related work. Conclusions are provided in Section~\ref{conclusion}.






